Information-theoretic generalization bounds for black-box learning algorithms

We derive information-theoretic generalization bounds for supervised learning algorithms based on the information contained in predictions rather than in the output of the training algorithm. These bounds improve over the existing information-theoretic bounds, are applicable to a wider range of algorithms, and solve two key challenges: (a) they give meaningful results for deterministic algorithms and (b) they are significantly easier to estimate. We show experimentally that the proposed bounds closely follow the generalization gap in practical scenarios for deep learning.

==> notes.tex <==
- Notational issues at the moment: We use the variable S in the two settings of Sec 2 differently.

*** DONE *** 

* General writing notes* 
- [+] which vs that
- [+] remove unnecessary colons before displaying math
- [+] punctuation
    - [+] Therefore, --> Therefore (in general if the phrase is short we don't want to put comma)
    - [+] be wary of commas before "such that"
    - [+] "we have:" -> "we have"
    - [+] be consistent with Oxford comma
    - [+] Then, -> Then

